Chasing the Clock: How Fast Are Vulnerabilities Fixed in the Maven Ecosystem?

This study investigates the software vulnerability resolution time in the Maven ecosystem, focusing on the influence of CVE severity, library popularity as measured by the number of dependents, and version release frequency. The results suggest that critical vulnerabilities are addressed slightly faster compared to lower-severity ones. Library popularity shows a positive impact on resolution times, while frequent version updates are associated with faster vulnerability fixes. These statistically significant findings are based on a thorough evaluation of over 14 million versions from 658,078 libraries using the dependency graph database of Goblin framework. These results emphasize the need for proactive maintenance strategies to improve vulnerability management in open-source ecosystems.

==> tables/MWW.tex <==
\begin{table}[htbp]
    \centering
    \small
       \vspace{-0.3cm}
    \caption{Pairwise Mann-Whitney-Wilcoxon test results for fix times}
    \vspace{-0.2cm}
    \label{tab:rq1SA}
    \setlength\tabcolsep{0.05pt}
     \begin{tabular}{|l|r|@{}c@{ }|l|r|}  \cline{1-2} \cline{4-5}
\textbf{Pair} & \textbf{p-value} & & \textbf{Pair} & \textbf{p-value} \\ \cline{1-2} \cline{4-5}
Critical vs High     & 0.0000 && High vs Moderate     & 0.0050  \\ \cline{1-2} \cline{4-5}
Critical vs Moderate & 0.0051 && High vs Low          & 0.7864 \\ \cline{1-2} \cline{4-5}
Critical vs Low      & 0.0213 && Moderate vs Low   & 0.3563\\ \cline{1-2} \cline{4-5}

   \end{tabular}
      % \vspace{-0.2cm}
\end{table}

